Top Couplings: pre-Snowmass Energy Frontier 2013 Overview

Overview on top couplings measurements is presented, and the prospects of future measurements are discussed. The coupling of top to the W boson can be examined either by looking at the decay of the top quark or from single top quark production. With the advent of high statistics top physics at the LHC and at the high-luminosity LHC, the processes where the bosons (photon, Z and Higgs) are produced in association with top quarks become accessible. The first evidence on the coupling of the top quark to these particles will come from the production rate.

==> Loginov/loginov_old.tex <==
The top quark was discovered almost twenty years ago. However,
couplings of the top quark to the electroweak (EW) gauge bosons have
not yet been directly measured. Due to the large mass, the top quark
may play a special role in EW symmetry breaking (EWSB), and therefore new
physics connected with EWSB can manifest itself in top precision
observables. Possible signals for new physics are deviations of the
$\ttbar\gamma$, $\ttbar Z$ and $tbW$ couplings from the values
predicted by the Standard Model (SM).

The $\ttbar \gamma$ and $\ttbar Z$ couplings cannot be constrained via
measurements of $\ttbar$ production at hadron colliders via
intermediate virtual $\gamma$ and $Z$ bosons, since the cross section
for $pp \rightarrow \ttbar$ is dominated by processes involving QCD
couplings only. The $tbW$ coupling may be constrained via measurements
of the single top quark production cross section. However, the $\ttbar
\gamma$ or $\ttbar Z$ couplings may be measured via
analysis of direct production of $\ttbar$ pairs in association with a
$\gamma$, $Z$ boson, respectively. The production of $\ttbar$ pairs
in association with a $W$ boson is a similar class of process, even though  
the $W$ does not couple to the top quark.

\subsection{$\ttbar+\gamma$}

The coupling to photons is sensitive to the electric charge of the top
quark. The charge of the top quark has been measured at both the
Tevatron and LHC using the track charge method (a weighted sum of the
charges of tracks associated with the $b$-jet) and the soft lepton
method (charge of the muon produced in the semi-leptonic decay
$b\rightarrow\mu\nu+X$ is defined by the $b$-quark charge).

Radiative $\ttbar$ production can be classified into the radiative top
quark production and radiative top quark decay, as shown in
Fig.~\ref{f:ttgamma_diagrams}.

\begin{figure}[htbp]
  \begin{center}
    \mbox{
\subfigure[Radiative top quark production]{\includegraphics[width=0.152\textwidth]{\home/Loginov/tty_prod_1}\hspace{0.12cm}\includegraphics[width=0.152\textwidth]{\home/Loginov/tty_prod_2}\hspace{0.12cm}\includegraphics[width=0.152\textwidth]{\home/Loginov/tty_prod_4}}
      }
    \mbox{
\subfigure[Radiative top quark decay]{\includegraphics[width=0.162\textwidth]{\home/Loginov/tty_dec_1}\includegraphics[width=0.162\textwidth]{\home/Loginov/tty_dec_2}\includegraphics[width=0.162\textwidth]{\home/Loginov/tty_dec_3}}
      }
    \caption {
Representative Feynman diagrams for the $\ttg$ process. }
    \label{f:ttgamma_diagrams}
  \end{center}
\end{figure}

The distinction between the two classes of processes is required for
determination of couplings of the top quark to the photon as discussed
below. However, the analyses performed so far by CDF and ATLAS
collaborations didn't measure the couplings, providing instead 
measurements of the $\ttbar\gamma$ cross section, $\sigma_{\ttg}$. In both the CDF and
ATLAS $\ttbar\gamma$ analyses the strategy is to perform data-driven
background estimates for jets misidentified as electrons, and for jets
and electrons misidentified as photons. In addition, $\ttbar$ and
$W\gamma$ production are used as control samples for the $\ttbar$ part
of the event and for the photons, respectively. Both $Z\rightarrow ee$
and $Z\rightarrow ee,~e\rightarrow\gamma$ are used to perform photon
identification studies and optimizations.

The CDF collaboration published the first experimental evidence for
$\ttg$ production by measuring $\sigma_{\ttg}$ and the ratio
$R=\sigma_{\ttg}/\sigma_{\ttbar}$ with data corresponding to 6.0~fb$^{-1}$ 
of $\ppbar$ collisions at $\sqrt{s}=1.96$ TeV at the
Tevatron. The $\ttg$ cross section was measured to be $\sigma_{\ttg} =
0.18 \pm 0.08$ pb for a photon $p_T > 10$ GeV, with a significance of
3.0~$\sigma$~\cite{cdf_ttgamma}. The ratio was measured to be $R =
0.024 \pm 0.009$ in a good agreement with the SM expectation of $0.024
\pm 0.005$ for a charge 2/3 top quark.

The ATLAS collaboration has performed the first $\ttbar\gamma$
production~\cite{atlas_ttgamma} cross section measurement at the LHC
with a photon $p_T$ threshold of 8 GeV in 1.04 fb$^{-1}$ of data at
$\sqrt{s}=7$ TeV, $\sigma_{\ttbar\gamma}=2.0\pm 0.5~(stat.)\pm
0.7~(syst.)\pm 0.8~(lumi.)$~pb. The significance of the
measurement is 2.7 $\sigma$, and the measured cross section is in
good agreement with the SM expectation of $2.1\pm 0.4$ pb for a charge
2/3 top quark. The analysis is being updated with the full 7 TeV
statistics.

The LO $\ttbar\gamma$ production cross section will increase by a
factor of 5 from 7 TeV to 14 TeV center-of-mass energy for photons
with $p_T>20$~GeV~\cite{Stelzer:1994ta,Maltoni:2002qb}. With a much larger statistics
expected after the upcoming 2013-2014 shutdown, analysis of the top
quark--photon couplings will be possible.

To isolate events with photon emission from top quarks, photon
radiation from the $W$ and its decay products, as well as from $b$ quarks
and from initial-state quarks should be suppressed, as detailed in
Ref.~\cite{tt_couplings_baur}. To suppress photon radiation from the
$b$ quarks (leptons) a large $\Delta R(\gamma,b)$ ($\Delta
R(\gamma,\ell)$) is required. Photon emission from $W$ decay products
can essentially be eliminated by requiring that the invariant mass of
the $jj\gamma$ system $m(jj\gamma) > 90~{\rm GeV}$ and the
$\ell\gamma\sla{p}_T$ cluster transverse mass
$m_T(\ell\gamma;\sla{p}_T) > 90~{\rm GeV}$. The radiation from the
initial state quarks is hard to suppress without simultaneously
reducing the signal cross section. However, as at the LHC the gluon
fusion $\ttbar$ production dominates, it is not an issue unlike at the
Tevatron. In addition, the event is required to be consistent either
with $\ttbar\gamma$ production, or with $\ttbar$ production with
radiative top decay by performing top quark and top quark + photon
mass reconstruction as shown in Ref.~\cite{tt_couplings_baur}.

Isolating events with photon emission from top quarks, as well as
performing a ratio $R=\sigma_{\ttg}/\sigma_{\ttbar}$ measurement to
reduce systematic uncertainties is the strategy for future
$\ttbar\gamma$ analyses. Detailed study of the $\ttbar\gamma$ final
state will be performed by measuring differential cross section (for
instance, as a function of photon $p_T$). The $\ttbar\gamma$ signature
is also a control sample for $\ttbar Z$ and $\ttbar
H,~H\rightarrow\gamma\gamma$ analyses.

\subsection{$\ttbar+W$,$\ttbar+Z$}

Representative Feynman diagrams for $\ttbar Z$ production are shown in
quark production and radiative top quark decay, as shown in
Fig.~\ref{f:ttz_diagrams}. The associated production of $\ttbar$ and
$Z$ (or $W$) bosons has been measured by CMS in 5 fb$^{-1}$ of pp
collisions at $\sqrt{s}=7~$TeV~\cite{ttv_cms}. An exclusive measurement
of the $\ttbar Z$ cross section $\sigma_{\ttbar Z} = 0.30
\pm{0.14}{0.11} (stat) \pm{0.04}{0.02} (syst)$ pb is obtained with a
significance of 3.66 $\sigma$ using trilepton events, observing 9
events with the expected background of 2.9 $\pm$ 0.8 events. The
significance of the $\ttbar V$ signal ($\ttbar Z$, $\ttbar W$) is
4.67 $\sigma$, and the combined $\ttbar V$ ($V$ = $Z$, $W$) cross
section is measured to be $\sigma_{\ttbar V} = 0.51 \pm{0.15}{0.13}
(stat) \pm{0.05}{0.04} (syst)$ pb using same-sign dileptons. The
signatures exploit the fact that SM events with two prompt same-sign
isolated leptons in the final state as well as trilepton events are
very rare. A data-driven estimation procedure is employed to estimate
the contribution of jets misidentified as leptons. The results are
shown in Figure~\ref{fig:ttv} together with the SM predictions.

\begin{figure}[!htbp]
  \centering
    \includegraphics[bb = 73 110 555 275,clip=,width=0.53\textwidth]{\home/Loginov/ttz_diagrams.ps}
    \caption{Representative Feynman diagrams for the $\ttbar Z$ process.}
    \label{f:ttz_diagrams}
\end{figure}

The ATLAS collaboration also performed $\ttbar Z$
analysis~\cite{ttz_atlas}, using a much tighter selection to suppress
backgrounds, that resulted in observing one event in data and setting
a limit $\sigma_{\ttbar Z} < 0.71~pb$ at 95\% CL consistent with the
CMS measurement and with theoretical predictions~\cite{ttz_baur}.

\begin{figure}[!thb]
\centerline{\epsfxsize=4.0in\epsfbox{\home/Loginov/ttV_cms.eps}}
\caption[*]{ Measurement of the $\ttbar V$ production cross
section~\cite{ttv_cms}: the cross section from the trilepton channel (blue
triangle), from the same sign dilepton channel (grey square) and the
combination of the two measurements (black circle) are compared to
the NLO calculation (red line). Internal error bars for the
measurements represent the statistical component of the uncertainty.}
\label{fig:ttv}
\end{figure}

With the current dataset the uncertainty of the $\ttbar V$ 
measurement is dominated by statistics. The LO $\ttbar V$ production
cross section will increase by an order of magnitude from 7 TeV to 14
TeV center-of-mass energy~\cite{Stelzer:1994ta,Maltoni:2002qb}, therefore providing
sufficient data for precise measurements of the $\ttbar V$ couplings
after the 2013-2014 shutdown.

